Dashboard Mechanisms for Online Marketplaces

This paper gives a theoretical model for design and analysis of mechanisms for online marketplaces where a bidding dashboard enables the bid-optimization of long-lived agents. We assume that a good allocation algorithm exists when given the true values of the agents and we develop online winner-pays-bid and all-pay mechanisms that implement the same outcome of the algorithm with the aid of a bidding dashboard. The bidding dashboards that we develop work in conjunction with the mechanism to guarantee that bidding according to the dashboard is strategically equivalent (with vanishing utility difference) to bidding truthfully in the sequential truthful implementation of the allocation algorithm. Our dashboard mechanism makes only a single call to the allocation algorithm in each stage.

==> a_proofs.tex <==

\section{Proofs from \Cref{s:no-regret}}
\label{a:proofs}






\begin{numberedtheorem}{\ref{thm:avebidbound}}
Suppose that a given player $i$ in the dashboard mechanism with an all-pay payment rule
and the allocation rule with derivative of
at least $1/(\alpha^2v^3)$ which is incentive
consistent on average and where bidder 
has regret within $[0,\,\overline{\regreti}]$.
Then 
\begin{enumerate}
\item The rationalizable values are within
$[v_i \pm 2\overline{\regreti}/\alpha]$, i.e.
if the average regret $\overline{\regreti}$
is decreasing, then the mechanism allocates
correctly for this bidder in the limit.
\item The average bid (corresponding
to the average payment in the all-pay mechanism) is bounded by
$$
\left|
\overline{\bidi^{(t)}}-\frac{1}{t}\sum\limits_{s \leq t}\bidi^{(s)}
\right| \leq \overline{\regreti}\left(
1+\frac{\alpha}{(v_i
-\overline{\regreti}/\alpha)^2}
\right)
$$
from the optimal fixed bid in hindsight $\overline{\bidi^{(t)}}$. I.e. if the average regret $\overline{\regreti}$
is decreasing, then the average payment
in the mechanism in the limit minimizes
regret of the bidder.
\end{enumerate}
\end{numberedtheorem}



\begin{proof}
 The lowest point of the rationalizable
set is the point of tangency of that set 
with the horizontal line. That line
corresponds to bid $\bidi^{(t)*}$ such that
$$
\frac{1}{t}\sum\limits_{s \leq t}
\balloci \super s \left(\bidi^{(t)*}\right)=
\frac{1}{t}\sum\limits_{s \leq t}\balloci^{(s)}(\bidi^{(s)}).
$$
Therefore, the value that rationalizes the lowest regret is
$$
\vali^{(t)*}=1/\frac{1}{t}\sum\limits_{s \leq t}\balloci^{\prime(s)}(\bidi^{(t)*})
$$
and the lowest regret is equal to
$$
\regreti^{(t)*}=\frac{1}{t}\sum\limits_{s \leq t}\bidi^{(s)}-\bidi^{(t)*}.
$$

Suppose that $\overline{\regreti}$ is bound
on regret for player $i$. Then by Lemma \ref{RS:boundary} (strong convexity of the 
rationalizable set) the range of
values that rationalize the history
of bidds of player $i$ is
$[\vali^{(t)*} \pm \overline{\regreti}/\alpha]$. This means
that for agent's true value
$|\vali-\vali^{(t)*}| \leq  \overline{\regreti}/\alpha$. 



The bound on regret implies that 
$\regreti^{(t)*} \leq \overline{\regreti}$.
As a result, in the average bid of the 
of the bidder with bounded regret is
within $\overline{\regreti}$ from the 
best $\bidi^{(t)*}$:
$$
\frac{1}{t}\sum\limits_{s \leq t}\bidi^{(s)} \leq \bidi^{(t)*}+\overline{\regreti}.
$$
Then if $\overline{\bidi^{(t)}}$ is the fixed
bid in hindsight that minimizes regret, then 
by Lemma \ref{l:strictly-monotone}, it follows that 
\begin{equation*}
\frac{|\bidi^{(t)*}-\overline{\bidi^{(t)}}|}{\alpha^2}\leq \left|\frac{1}{t}\sum\limits_{s \leq t}
\balloci^{\prime (s)} \left(\bidi^{(t)*}\right)-
\frac{1}{t}\sum\limits_{s \leq t}
\balloci^{\prime (s)} \left(\overline{\bidi^{(t)}}\right)\right|
=\left|
\frac{1}{\vali}-\frac{1}{\vali^{(t)*}}
\right| \leq \frac{\overline{\regreti}/\alpha}{(v_i
-\overline{\regreti}/\alpha)^2}.
\qedhere
\end{equation*}
\end{proof}










\begin{numberedtheorem}{\ref{thm:avepayminreg}}
Suppose that a given player in the dashboard mechanism with a winner-pays-bid payment rule
and the allocation rule with log-derivative of
at least $1/\alpha^2v^3$ which is incentive
consistent on average and where bidder 
has regret within $[0,\,\overline{\regreti}]$.
Then 
\begin{enumerate}
\item The range of values that rationalizes
bids of this bidder is contained in $[v_i \pm 2 \overline{\regreti}/\alpha]$. In other words, if the bidder has vanishing regret, then the mechanism allocates this bidder
correctly in the limit.
\item The average payment per unit of allocation can be bounded as
$$
\left|
\overline{\bidi^{(t)}}-\frac{\frac{1}{t}\sum\limits_{s \leq t}\bidi \super s \balloci \super s (\bidi \super s)}
 {\frac{1}{t}\sum\limits_{s \leq t}\balloci \super s (\bidi \super s)}
\right| \leq \frac{\overline{\regreti}}{
\alpha^2v_i-\alpha\overline{\regreti}}\left(
1+\frac{\alpha^3}{v_i
-\overline{\regreti}/\alpha}
\right)
$$
from the optimal fixed bid in hindsight $\overline{\bidi^{(t)}}$. In other words,
the average payment of this bidder in the 
limit minimizes regret.
\end{enumerate}
\end{numberedtheorem}

\begin{proof}
The upper bound of $\epsilon_i$ for the average regret leads to the rationalizable
set of values and average regrets. The value that rationalizes the smallest regret
is induced by bid $\bidi^{(t)*}$
\begin{equation}\label{alloc:eq}
\sum\limits_{s \leq t}\balloci^{(s)}(\bidi^{(t)*})=\sum\limits_{s \leq t}\balloci^{(s)}(\bidi^{(s)}).
\end{equation}
Then the value that rationalizes the smallest regret is
$$
\vali^{(t)*}(b)=\bidi^{(t)*} + \frac{1}{t}\sum\limits_{s \leq t}\balloci \super s (\bidi^{(t)*})
    \bigg/
    \frac{1}{t}\sum\limits_{s \leq t} \balloci^{\prime (s)}(\bidi^{(t)*})
$$
The lowest regret is equal to 
$$
\regreti^{(t)*}=\frac{1}{t}\sum\limits_{s \leq t}\bidi \super s \balloci \super s (\bidi \super s)-
\bidi^{(t)*}\frac{1}{t}\sum\limits_{s \leq t}\balloci \super s (\bidi^{(t)*})
$$


Suppose that $\overline{\regreti}$ is bound
on regret for player $i$. Then by Lemma \ref{RS:boundary:FPA} (strong convexity of the 
rationalizable set) the range of
values that rationalize the history
of bidds of player $i$ is
$[\vali^{(t)*} \pm \overline{\regreti}/\alpha]$. This means
that for agent's true value
$|\vali-\vali^{(t)*}| \leq  \overline{\regreti}/\alpha$. This result is identical to the bound for the rationalizable
values in the all-pay mechanism.

The bound on regret leads to $\regreti^{(t)*}
 \leq \overline{\regreti}$. In light
 of (\ref{alloc:eq}), this means that 
 $$
 \frac{1}{t}\sum\limits_{s \leq t}\balloci \super s (\bidi^{(t)*}) \left(\frac{\frac{1}{t}\sum\limits_{s \leq t}\bidi \super s \balloci \super s (\bidi \super s)}
 {\frac{1}{t}\sum\limits_{s \leq t}\balloci \super s (\bidi \super s)}-
\bidi^{(t)*}\right)
\leq \overline{\regreti}.
$$
 Then
 $$
 \frac{1}{t}\sum\limits_{s \leq t}\balloci \super s (\bidi^{(t)*}) \geq \alpha^2 \vali^{(t)*}. $$
As a result
$$
\frac{\frac{1}{t}\sum\limits_{s \leq t}\bidi \super s \balloci \super s (\bidi \super s)}
 {\frac{1}{t}\sum\limits_{s \leq t}\balloci \super s (\bidi \super s)}-
\bidi^{(t)*} \leq \frac{\overline{\regreti}}{
\alpha^2v_i-\alpha\overline{\regreti}}
$$
By strong convexity of the utility 
function it follows that the optimal fixed
bid in hindsight can be bounded as
\begin{equation*}
|\bidi^{(t)*} -\overline{\bidi \super t}|
 \leq \frac{\alpha \overline{\regreti}}{(v_i- \regreti/\alpha)^2}
 \qedhere
\end{equation*}
\end{proof}

==> extra_notes.tex <==
\section{Attempts at Winner-pays-bid}

Consider a (value) allocaction rule $\alloc$ that is arbitrary up to
$V$ and linear with slope $\alloc'(\val) = \delta$ at $\val \geq V$.
Define allocation $X = \alloc(V)$, price $P = \price(V)$, and bid $B =
P/X$ at $\val = V$. For $\val = V + \nu \geq V$ write $\alloc_V(\nu) = \alloc(V  + \nu)$ we have:
\begin{align*}
\alloc_V(\nu) & = X + \delta \nu,\\
\price_V(\nu) & = P + \delta \nu (V + \nu/2),\\
\bid_V(\nu) &= \frac{P + \delta V \nu + (\delta / 2) \nu^2}{X + \delta \nu}\\
%
\intertext{We would like to find $\balloc_B(\beta) = \balloc(B +
  \beta)$ with $\balloc_B(\bid_V(\nu)) = \alloc_V(\nu)$ and understand
  its slope in terms of $\delta$}
%
\balloc_B(\beta) &= \alloc_V(\bid_V^{-1}(B+\beta))
\end{align*}
The idea is that $\alloc$ is linear, $\price$ is quadratic, $\bid$ is
the ratio of a quadratic to a linear, which should be approximately
linear, so its inversion should be approximately linear, so plugging
in the inverse into $\alloc$ which is linear, will be linear and the
coefficient is the product of the coefficients.

If you just drop the lower order terms you get $\balloc'_B(\beta) = 2
\delta$.  I'm unsure of how to properly do this analysis.


\underline{Direct approach:} Let's find the inverse $\bid_V^{-1}(\cdot)$ at $B+\beta$ directly,
i.e. solve for $\nu$ such that 
$$
B+\beta=\frac{P + \delta V \nu + (\delta / 2) \nu^2}{X + \delta \nu},
$$
taking into account that $B=P/X$. Then 
$$
(B+\beta)(X+\delta \nu)=P+X\beta+\delta \nu(B+\beta).
$$
This produces the following quadratic equation 
$$
\frac{\delta}{2}\nu^2+\delta\nu (V-B-\beta)-X\beta=0.
$$
This equation has two roots one of which is negative and we can drop it. The positive one is
$$
\nu_{\beta}=\sqrt{(V-B-\beta)^2+\frac{2\beta X}{\delta}}-(V-B-\beta).
$$
Assume that $\beta$ is infinitesimal and produce an approximation for $\nu_{\beta}$ up to terms
of order $o(\beta)$ as follows
\begin{align*}
\nu_{\beta}=(V-B-\beta)\sqrt{1+\frac{2\beta X}{(V-B-\beta)^2\delta}}-(V-B-\beta)
\end{align*}
In this expression
\begin{align*}
&\frac{2\beta X}{(V-B-\beta)^2\delta}=\frac{2\beta X}{(1-2\frac{\beta}{V-B}+\frac{\beta^2}{(V-B)^2})(V-B)^2\delta}\\
&=\frac{2\beta X}{(1-2\frac{\beta}{V-B}+o(\beta))(V-B)^2
\delta}=
\frac{2X}{(V-B)^2 \delta}\beta(1+2\frac{\beta}{V-B}+o(\beta)),
\end{align*}
where the last expression follows from the evaluation $1/(1-x)=1+x+o(x)$ as $x \rightarrow 0$.
Then 
$$
\frac{2\beta X}{(V-B-\beta)^2\sqrt{\delta}}=\frac{2X}{(V-B)^2 \delta}\beta+o(\beta)
$$
As a result
$$
\sqrt{1+\frac{2\beta X}{(V-B-\beta)^2\delta}}=1+\frac{X}{(V-B)^2 \delta}\beta+o(\beta),
$$
which follows from the evaluation $(1+x)^{\alpha}=1+\alpha x +o(x)$ as $x \rightarrow 0$. Then
$$
\nu_{\beta}=\frac{X}{V-B}\,\frac{\beta}{
\delta}+o(\beta)
$$
As a result,
$$
\alloc_V(\nu_{\beta})  = X + \frac{X}{V-B}\,\beta+o(\beta),
$$
and the derivative of the bid allocation rule is
$$
\balloc_B'(b)= \lim\limits_{\beta \rightarrow 0}\frac{\alloc_V(\nu_{\beta})-X}{\beta}=\frac{X}{V-B}
$$


\paragraph{Jason's addition}

From above:
\begin{align*}
\nu(\beta)&=\sqrt{(V-B-\beta)^2+\frac{2\beta X}{\delta}}-(V-B-\beta),\\
\nu'(\beta)&=\frac{2(V-B-\beta)(-1) + 2X/\delta}{2\sqrt{(V-B-\beta)^2+\frac{2\beta X}{\delta}}} + 1\\
   &=\frac{X/\delta - (V-B-\beta)}{\sqrt{(V-B-\beta)^2+\frac{2\beta X}{\delta}}} + 1.\\
\intertext{With $\balloc(B + \beta) = X + \delta\nu(\beta)$ we have}
\balloc'_B(\beta) &= \delta \nu'(\beta)\\
                  &=\frac{X - \delta(V-B-\beta)}{\sqrt{(V-B-\beta)^2+\frac{2\beta X}{\delta}}} + \delta.\\
\intertext{Notice that if $\alloc'(\val) > \delta$ (everywhere) then $X \geq \delta V$ so the first term is non-negative.  We have:}
\balloc'_B(\beta) & \geq \delta.
\end{align*}


==> fictitious.tex <==
\section{Implementation in Fictitious Play}

\label{s:fictitious}

In this section we consider the dashboard mechanism with a dashboard
that corresponds to the empirical bid allocation rule.  Agents who bid
according to such a dashboard are engaging in the standard solution
concept of fictitious play.  For any monotone strictly continuous
social choice function, we will give a mechanism that implements the
social choice function in fictitious play.  Moreover, under an
assumption on the smoothness of the resulting bid-allocation rules, in
the limit of fictitious play the bids converge to a Nash equilibrium
in the stage mechanism.  Consequently, the corresponding
fictitious-play dashboard mechanism implents the social choice
function for persuadable agents.

Informally, fictitious play suggests that an agent in stage $t+1$ will
act in best response to the empirical distribution of actions of
agents in previous stages.  Denote bid profile in stage $t$ by $\bids
\super t$.  Denote the bid allocation rule of a mechanism in stage $t$
by $\ballocs \super{t} : \reals^n \to [0,1]^n$.  The profile of
empirical allocation rules is $\eballocs\super t \in (\reals \to
[0,1])^n$ given by $\eballoci^{(t)}(\bidi) = \frac{1}{t} \sum_{s \leq
  t} \balloci(\bidi,\bidsmi\super s)$ for each agent $i$.
Specifically, the empirical bid allocation rule for an agent $i$ is
calculated by fixing the historical bids of other agents
$\bidsmi\super 1,\ldots,\bidsmi\super t$ and replaying history with a
new bid $\bidi$ for agent $i$.  The history in stage $t+1$ is
$\bids\super 1,\ldots,\bids\super t$.  In Internet market places, the
most appropriate interpretation of fictitious play suggests that the
bids in stage $t+1$ are best responses to the empirical allocation
rules for stages $1$ through $t$, namely $\eballocs\super t$.
Moreover, a market maker can encourage agents to optimize thus by
publishing the each agent's empirical allocation rule as part of the
agent's bidding dashboard.

\begin{definition}
Agents with values $\vals$ in stage $t+1$ of {\em fictitious play} bid
in best response to the profile of empirical allocation rules
$\eballocs^{(t)}$.  Specifically, each agent $i$'s bid satisfies
$\bidi^{(t)} \in \argmax_z (\vali -
z)\,\eballoci^{(t)}(z)$.\footnote{This definition assumes a
  winner-pays-bid mechanism, it could be extended for general
  mechanisms by explicitly defining the profile of empirical payment
  rules.}
\end{definition}

Notice that if the empirical allocation rule of each agent is
continuous and strictly increasing then the agent's value can easily
be determined from her bid.  The optimal bid $\bidi^{(t)}$ for agent
$i$ at stage $t$ with empirical allocation rule $\eballoci$ solves
$\ddx{z} (\vali - z)\, \eballoci^{(t)}(z) = 0$; thus, the value of
agent $i$ can be calculated as:
$$
\evali^{(t)} = \bidi + \eballoci^{(t)}(\bidi)/\eballoci^{\prime (t)}(\bidi)
$$ 
where $\eballoci^{\prime (t)}(z) = \ddx{z} \eballoci^{(t)}(z)$.  We
refer to this value as the {\em estimated value} for the agent.


The definition of fictitious play above allows the mechanisms run at each
stage, denoted $\ballocs^t$, to be distinct.  Specifically, the
mechanism we suggest is one where the market maker parameterizes the
mechanism in stage $t+1$ by the profile of empirical allocation rules
(i.e., from the bids in previous stages). The goal of this
mechanism is to implement social choice rule $\allocs : \reals^n \to
[0,1]^n$.

\begin{definition} 
\label{d:fictitious-play-mech}
The winner-pays-bid implementation of social choice rule $\allocs$ in
fictitious play for stage $t+1$ is:
\begin{enumerate}
\item[0.] \label{fictitious-play-mech:solicit}
Solicit bids $\bids$ that are best responses to the profile
  of empirical allocation rules $\eballocs^{(t)}$.
\item \label{fictitious-play-mech:estimate}
Estimate the value $\evali^{(t)}$ of each agent $i$ from her empirical
  allocation rule $\eballoci \super t$ and bid $\bidi \super t$.
\item \label{fictitious-play-mech:execute}
Execute the social choice function $\allocs$ on the estimated
  values $\evals^{(t)}$ to determine the outcome; charge each winner her
  bid.
\end{enumerate}
\end{definition}

This mechanism admits the following analysis for social choice
functions where the allocation probability of each agent is continuous
and strictly increasing in her value.  In fictitious play, the
mechanism implements the social choice function.  
%Second, the bids of
%fictitious play converge to Nash equilibrium bids, i.e., matching the
%payment identity; namely $\lim_{t \to \infty} \bidi^t(\vali) =
%\pricei(\vals) / \alloci(\vals)$.  
The formal statement and proof of this observation conclude the
section.

\begin{prop}
\label{prop:fictitious-play-implementation}
For continuous and strictly increasing social choice rule $\allocs$,
the mechanism of Definition~\ref{d:fictitious-play-mech} implements
$\allocs$ in fictitious play.
\end{prop}

\begin{proof} 
Since the social choice rule is continuous and strictly increasing,
the agents' values uniquely determine their bids in
Step~\ref{fictitious-play-mech:solicit}, and are uniquely inverted to
give estimated values $\evals$ that equal the agents' values $\vals$
in Step~\ref{fictitious-play-mech:estimate}.
Step~\ref{fictitious-play-mech:execute}, then, produces the desired
outcome of the social choice rule.
\end{proof}


We now discuss asymptotic convergence of the empirical allocation rule 
$\eballoci^{(t)}$ as the number of periods $t$ increases. Given that the empirical
allocation rule uses the first-order condition of the agent in each period
to implement the allocation rule for the next period such a convergence 
can occur only when the class of allocation rules used to initialize and 
propagate the iterations of the fictitious play consists of sufficiently smooth 
functions. This requires additional stronger assumptions regarding the social
choice function $\allocs$ that guarantees such a smoothness on each stage.


\begin{definition}
Let $B$ be a bounded interval of the real line and $r$ a positive constant. 
By $\mcC(B,r)$ we define the $(1,\infty)$-Sobolev ball
of functions on $B$ of radius $r$, i.e. the space of functions $\varphi(\cdot)$ such that 
\begin{itemize}
\item for any function $f(\cdot)$ differentiable on $B$ there exists a {\it weak derivative} $\varphi'(\cdot)$
defined by $\int_B\varphi'(\beta)f(\beta)\,d\beta=-\int_B\varphi(\beta)f'(\beta)\,d\beta$;
\item function $\varphi(\cdot)$ and derivative $\varphi'(\cdot)$ are in ${\bf L}_{\infty}(B)$, the Lebesgue space with norm $\|z\|=\sup_b|z(b)|$; and
\item the {\it Sobolev norm} of $\varphi(\cdot)$ is bounded: $\|\varphi\|+\|\varphi'\|\leq r$.
\end{itemize}
\end{definition}

The definition of the Sobolev ball provides a sufficient condition for
the limit of sequence of the fictitous play to be unique as fomulated
in the following proposition.

\begin{prop}
Let $\eballocs^{(s)}$ for $s \leq t$ be the sequence of the empirical
bid allocation rules generated by the mechanism of
\Cref{d:fictitious-play-mech}. Suppose that for each $s$, $i$, and
$\evalsmi \super s$ functions $\eballoci^{(s)}(\cdot)$ are such that functions 
$$g(z) = \alloci\left(z
+\eballoci^{(s)}(z)/\eballoci^{\prime(s)}(z),\evalsmi \super s
\right)
$$
are contained in the Sobolev ball $\mcC([l,h],\,r)$ with $0 \leq l<h <1$.
Suppose also that functions $\alloci(\cdot,\evalsmi \super s)$ are Lipschitz
with universal Lipschitz constants $L_{1i}$ over $\evalsmi \super s$ and their inverses $\alloci^{-1}(\cdot,
\evalsmi \super s)$ are Lipschitz
with universal Lipschitz constants $L_{2i}$ such that for some small $\epsilon_i>0$, $L_{1i}
L_{2i}<1-\epsilon_i$. Then the mechanism of Definition~\ref{d:fictitious-play-mech} generates
the sequence of allocation rules that converges uniformly (over the bid space) to a unique limit
corresponding to the Nash equilibrium that induces the social choice function $\allocs$.
\end{prop}

\begin{proof}
We turn to the first-order condition of the agent that determines
the value $\evali$. In our further analysis we omit index $i$ since
it will be focused exclusively on the agent $i$ and the derivations for remaining agents
will be equivalent. Denote
$\logealloc \super t(b)=\log\,\eballoci \super t(b)$. In this case, the first-order condition for the 
agent takes the form
$
\evali\super t=b+1/\logealloc^{\prime (t)}(b).
$
Suppose that fictitious play is initialized using allocation function 
$\logealloc \super 0(\cdot)$. We can express the mapping that takes
the empirical allocation rule $\logealloc \super t$ and generates
the empirical allocation rule $\logealloc \super{t+1}$ as
\begin{equation}\label{FPM}
\textstyle \logealloc \super{t+1}(b)=\log\left(\frac{t}{t+1}e^{\logealloc \super t(b)}+\frac{1}{t+1}\alloci \super t
\left(
b+\frac{1}{\logealloc^{\prime (t)}(b)}
\right)\right)
\end{equation}
Thus, for the mapping defined as
$
M_{t+1}[z]=\log\left(\frac{t}{t+1}e^{z(b)}+\frac{1}{t+1}x
\left(
b+\frac{1}{z'(b)}
\right)\right)
$
we can re-write equation (\ref{FPM}) as
$
\logealloc \super{t+1}(b)=M_{t+1}[\logealloc \super t].
$
It is algebraically inconvenient to work with allocation functions
directly and instead consider functions $[0,1]\mapsto [0,1]$ such that
\begin{equation}\label{argument}
\varphi(b)=x\left(1/z'(b)+b \right),
\end{equation}
where  
$z\,:\,[0,\,1]\mapsto [0,\,1]$ are monotone increasing functions with $z(0)=0$ and
which have two 
continuous derivatives.


We now restrict the analysis to a specific class of functions that will be candidates for limit
of the average allocation rule resulting in the iterative process described above.


Knowing that the selected bids will be in some sufficiently small range, we take 
points $0 \leq l,\,h<1$ and consider allocation functions only on the interval $[l,\,h]$.
We now assume that functions $\varphi(\cdot)$ defined in (\ref{argument})
are in the Sobolev ball $\mcC([l,h],\,r)$.

Now we re-define mapping $M_{t+1}[\cdot]$ to operate on functions in $\mcC([l,h],\,r)$. Using the definition
of $\varphi(\cdot)$ we express the input of the mapping as
$
z(b)=\int^b_0\frac{d\beta}{x^{-1}(\varphi(\beta))-\beta}.
$
Mapping $M_{t+1}[\cdot]$ then can be written in terms of $\varphi$ and
$$ \textstyle
m_{t+1}[\varphi]=\log\left(\frac{t}{t+1}e^{\int^b_0\frac{d\beta}{x^{-1}(\varphi(\beta))-\beta}}+\frac{1}{t+1} \varphi(b)\right)
$$
Now we transform the outcome to ensure that we produce the mapping from the space of functions
$\varphi$ into itself. To do so we take
\begin{equation}\label{FPM:1}
\mu_{t+1}[\varphi]=
x
\left(
\frac{1}{\frac{d}{db}\mu_{t+1}[\varphi]}+b
\right)=
x\left(
\frac{
t e^{ \int^b_0\frac{d\beta}{x^{-1}(\varphi(\beta))-\beta}}+\varphi(b)
}{
\frac{t}{x^{-1}(\varphi(b))-b} e^{\int^b_0\frac{d\beta}{x^{-1}(\varphi(\beta))-\beta}}+\varphi'(b)}+b
\right)
\end{equation}


Take $\varphi_1,\varphi_2 \in \mcC([l,h],\,r)$ then evaluate
\begin{align*}
|&\mu_{t+1}[\varphi_1]-\mu_{t+1}[\varphi_2]| \leq L_1
\left|
\frac{
t e^{ \int^b_0\frac{d\beta}{x^{-1}(\varphi_1(\beta))-\beta}}+\varphi_1(b)
}{
\frac{t}{x^{-1}(\varphi_1(b))-b} e^{\int^b_0\frac{d\beta}{x^{-1}(\varphi_1(\beta))-\beta}}+\varphi'_1(b)}
-
\frac{
t e^{ \int^b_0\frac{d\beta}{x^{-1}(\varphi_2(\beta))-\beta}}+\varphi_2(b)
}{
\frac{t}{x^{-1}(\varphi_2(b))-b} e^{\int^b_0\frac{d\beta}{x^{-1}(\varphi_2(\beta))-\beta}}+\varphi'_2(b)}
\right|\\
 &\leq \frac{
1+\frac{1}{t} \varphi_1(b)e^{ -\int^b_0\frac{d\beta}{x^{-1}(\varphi_1(\beta))-\beta}}
}{
1+\frac{1}{t} (x^{-1}(\varphi_1(b))-b)\varphi_1'(b)e^{ -\int^b_0\frac{d\beta}{x^{-1}(\varphi_1(\beta))-\beta}}
}L_1L_2|\varphi_1(b)-\varphi_2(b)|\\
&+|x^{-1}(\varphi_2(b))-b|\bigg|
 \frac{
1+\frac{1}{t} \varphi_1(b)e^{ -\int^b_0\frac{d\beta}{x^{-1}(\varphi_1(\beta))-\beta}}
}{
1+\frac{1}{t} (x^{-1}(\varphi_1(b))-b)\varphi_1'(b)e^{ -\int^b_0\frac{d\beta}{x^{-1}(\varphi_1(\beta))-\beta}}
}\\
&\hspace{3in}-
 \frac{
1+\frac{1}{t} \varphi_2(b)e^{ -\int^b_0\frac{d\beta}{x^{-1}(\varphi_2(\beta))-\beta}}
}{
1+\frac{1}{t} (x^{-1}(\varphi_2(b))-b)\varphi_2'(b)e^{ -\int^b_0\frac{d\beta}{x^{-1}(\varphi_2(\beta))-\beta}}
}
\bigg|\\
&\leq \frac{
1+\frac{1}{t} \varphi_1(b)e^{ -\int^b_0\frac{d\beta}{x^{-1}(\varphi_1(\beta))-\beta}}
}{
1+\frac{1}{t} (x^{-1}(\varphi_1(b))-b)\varphi_1'(b)e^{ -\int^b_0\frac{d\beta}{x^{-1}(\varphi_1(\beta))-\beta}}
}L_1L_2|\varphi_1(b)-\varphi_2(b)|\\
&+
\frac{
\left(4\frac{L_1L_2 r}{t}+\frac{L_1L_2 r^2}{t^2}\right)|\varphi_1(b)-\varphi_2(b)|
}{
\left(1+
\frac{1}{t} (x^{-1}(\varphi_1(b))-b)\varphi_1'(b) e^{ -\int^b_0\frac{d\beta}{x^{-1}(\varphi_1(\beta))-\beta}}
\right)
\left(1+\frac{1}{t} (x^{-1}(\varphi_2(b))-b)\varphi_2'(b)e^{ 
-\int^b_0\frac{d\beta}{x^{-1}(\varphi_2(\beta))-\beta}}\right)
}
\\
\end{align*}
Given that $\varphi_1(\cdot),\varphi_2(\cdot) \in \mcC([l,h],\,r)$
(and, thus, $|\varphi_{1,2}'(\cdot)| \leq r$), for any $\alpha \in (0,\,1)$
there is large enough $T$ such that for all $T$
$$
\frac{
1+\frac{1}{t} (x^{-1}(\varphi_i(b))-b)\varphi_i'(b)e^{ -\int^b_0\frac{d\beta}{x^{-1}(\varphi_i(\beta))-\beta}}
}{
1+\frac{1}{t} \varphi_i(b)e^{ -\int^b_0\frac{d\beta}{x^{-1}(\varphi_i(\beta))-\beta}}
} \geq \alpha,\;\;i=1,2.
$$
The choice of $\alpha \geq 1-\epsilon/2$ ensures that the mapping of interest is a contraction mapping from $\mcC([l,h],r)$ into itself. This means that the limit of 
iterations defined by (\ref{FPM}) exists and it is unique. Given that we defined
the Sobolev ball using the norm in ${\bf L}_{\infty}([l,\,h])$, the sequence
of allocation rules $\eallocs \super t$ converges uniformly to a unique limit. Note that 
mapping of interest is characterized by (\ref{FPM:1}), the corresponding limit
implements $\alloc$.
\end{proof}

%% \begin{theorem}
%% \label{t:fictitious-play-limit}
%% For continuous and strictly increasing social choice rule $\allocs$
%% and the mechanism of Definition~\ref{d:fictitious-play-mech}, the bids
%% of fictitious play converge to the Nash equilibrium bids that
%% correspond to payment identity for $\allocs$ on the valuation profile
%% $\vals$.
%% \end{theorem}

%% \begin{proof}
%% ADD PROOF HERE.
%% \end{proof}



==> inconsistency.tex <==
%% In the next section we will show that the regret, in the learning
%% sense, of an agent that follows the dashboard in the last-stage
%% all-pay dashboard mechanism vanishes with the number of stages
%% $t$. Specifically, for any actions of the other agents, an agent with
%% value $\val$ that follows the dashboard has average stage utility that is
%% at least the average stage utility of any fixed bid in hindsight (up
%% to an additive loss of $\val/t$).


\section{Incentive Consistency, No-Regret, and the All-pay Last-stage Dashboard}
\label{s:inconsistency}

In this section we define a notion of incentive inconsistency that
will quantify as an additive loss how different are average utilities
obtained from strategies in dashboard mechanisms to those from
strategies in truthful mechanisms.  Outcomes from strategies with
vanishing incentive inconsistency will be analyzable via the usual
geometric understanding incentive compatible mechanisms in
single-dimensional environments from \citet{mye-81}.  The strategies
in the definition can be any perhaps randomized mapping from an
agent's value and observable histories to bids, as usual in an
extensive form game.

\begin{definition}
A dashboard mechanism is $\epsilon$ {\em incentive inconsistent for an
  agent strategy} if, for any induced allocation rules $\alloc \super
1,\ldots,\alloc \super t$ of the mechanism, an agent strategy
generates a sequence of bids $\bid \super 1, \ldots, \bid \super t$
that imply inferred values $\eval \super 1,\ldots,\eval \super t$ for
which the average per-stage outcomes satisfy
\begin{align*}
\frac{1}{t}\sum\nolimits_{s=1}^t \balloc \super s (\bid \super s) &=
\frac{1}{t}\sum\nolimits_{s=1}^t \alloc \super s (\eval \super s), &
\frac{1}{t}\sum\nolimits_{s=1}^t \bprice \super s (\bid \super s) &=
\frac{1}{t}\sum\nolimits_{s=1}^t \price \super s (\eval \super s) \pm
\epsilon.
\end{align*}
If this condition holds for all strategies, the dashboard is {\em
  $\epsilon$ incentive inconsistent}.  A dashboard is {\em incentive
  consistent} if its incentive inconsistency vanishes with the number
of stages $t$.
\end{definition}

A consequence of $\epsilon$ incentive inconsistency is that the
(value) allocation rules induce agent utility as they usually do in
Nash equilibrium.  Specifically, denote by $\util(\val,\eval) = \val\,
\alloc(\eval) - \price(\eval)$ the utility of an agent with value
$\val$ following the dashboard optimally for an agent with value
$\eval$.

\begin{lemma}
\label{l:utility-under-incentive-consistency}
If the dashboard mechanism is $\epsilon$ incentive inconsistent with the
agent strategy then the agent with values $\val\super s$ in each stage $s$ and inferred values according to the strategy of $\eval \super s$ in each stage $s$ has utility
\begin{align}
\label{eq:util-ii}
\frac{1}{n}\sum\nolimits_{s=1}^t \util \super s (\val \super s,\eval \super s) \pm \epsilon
\end{align}
\end{lemma}
\begin{proof}
From the definitions of utility and incentive inconsistency.
\end{proof}

In this section we will focus on two particular kinds of strategies.
In the {\em follow-the-dashboard} strategy an agent with value $\val$
bids optimally for her value and the given dashboard $\dalloc$.  In
the {\em constant-bid} strategy an agent bids a fixed bid $\bid$ in
every stage.  The following theorem shows that following the dashboard
is a no-regret strategy.

%The following two propositions motivate the definitions
%of incentive inconsistency.
%
%\begin{theorem}
%If a dashboard is $\epsilon$ incentive inconsistent (for all
%strategies), then the follow-the-dashboard strategy is an
%$\epsilon$-Nash equilibrium.
%\end{theorem}

%\begin{proof}
%\end{proof}

\begin{theorem}
If a dashboard is $\epsilon_{\FTD}$ and $\epsilon_{\CB}$ incentive
inconsistent for the follow-the-dashboard strategy and all
constant-bid strategies, respectively, then the
following-the-dashboard strategy has regret at most $\epsilon_{\FTD} +
\epsilon_{CB}$.
\end{theorem} 

\begin{proof}
Consider the follow-the-dashboard strategy and fix the resulting
sequence of stage allocation rules.  We compare the utility of
following the dashboard to any fixed bid in hindsight (where ``in
hindsight'' means with respect to the stage allocation rules resulting
from the follow-the-dashboard strategy).  

Write the utility of the agent in stage $s$ with value $\val$ and
estimated value $\eval$ in the incentive compatible mechanism with
allocation rule $\alloc \super s$ as: 
\begin{align}
\label{eq:ic-util}
\util \super s (\val,\eval) &=
\val \alloc \super s(\eval) - \price \super s(\eval).\\
\intertext{Incentive compatibility requires for all $\eval$ that the true value gives $\val$ higher utility than $\eval$}
\label{eq:ic-util-ineq}
\util \super s (\val,\val) & \geq \util \super s (\val,\eval).
\end{align}


The inferred values for the follow-the-dashboard strategy are
identically $\val$.  Denote the inferred values for the constant-bid
strategy as $\eval \super 1,\ldots,\eval \super t$.  Denote the
agent's average stage utility from following the dashboard by
$\util_{\FTD}$ and the utility from the constant bid by $\util_{\CB}$.
The definition of incentive inconsistency, definition of
utility~\eqref{eq:ic-util}, and truth-telling utility inequality
\eqref{eq:ic-util-ineq} give:
\begin{align*}
\util_{\FTD} 
   &\geq \frac{1}{t} \sum\nolimits_s \util \super s (\val,\val) - \epsilon_{\FTD}\\
   &\geq \frac{1}{t} \sum\nolimits_s \util \super s (\val,\eval \super s) - \epsilon_{\FTD}\\
   &\geq \util_{\CB} - \epsilon_{\FTD} - \epsilon_{CB}. \qedhere
\end{align*}
\end{proof}

Below we show that the all-pay last-stage dashboard (\Cref{d:last-stage}) is incentive
consistent for follow-the-dashboard and constant-bid strategies.  A
key observation that makes the incentive consistency straightforward
in all-pay last-stage dashboard mechanism is that the payment in stage
$s+1$ is the correct incentive compatible payment for the allocation
of stage $s$. Thus, pairing as ``outcome $s$'' the allocation from
stage $s$ with the payment from stage $s+1$, we may as well view the
outcomes as those from a sequence of incentive compatible mechanisms
when averaging across $t$ stages (up to a vanishing loss of at most
$\val/t$ for the one stage that cannot be paired like this).

The lemmas below show that all-pay last-stage dashboard is $\epsilon$
incentive inconsistent with for both the strategy of following the
dashboard for any fixed value $\val$ and the strategy of bidding any
fixed bid $\bid$.  For the former $\epsilon \leq \val/t$; for the
latter $\epsilon = 0$.


\begin{lemma} 
\label{l:follow-the-dashboard-incentive-consistency}
For an agent with static per-stage value $\val$, 
the last-stage all-pay dashboard is $\val/t$ incentive inconsistent
for the follow-the-dashboard strategy.
\end{lemma} 

\begin{proof}
We will consider grouping the allocation of stage $s$ with the payment
in stage $s+1$ (with the allocation of round $t$ paired with the
payment of round $1$) and we will refer to this grouping as outcome
$s$.  As we have discussed above, if the agent follows the dashboard,
outcomes corresponding to $s \in \{1,\ldots,t-1\}$ are incentive
compatible outcomes for the allocation rule of stage $s$ and value
$\val$.  The imbalance of payments from outcome $t$ (allocation from
stage $t$ and payment from stage 1; for formal argument see
\Cref{l:maximum-imbalance} in \Cref{s:rebalancing}) is at most $\val$.
\end{proof}

\begin{lemma}
The last-stage all-pay dashboard is $0$ incentive inconsistent
for the constant bid strategy.
\end{lemma} 


\begin{proof}
THIS LEMMA IS INCORRECT.
 
For fixed stage allocation rules, consider the hindsight deviation of
an agent to bid $\bid\primed$ in every stage, similarly grouping
allocations and payments into outcomes as in the proof of
\Cref{l:follow-the-dashboard-incentive-consistency}, the outcome in
stage $s \in \{1,\ldots,t\}$ are incentive compatible outcomes for the
allocation rule of stage $s$ and the value $\eval \super s$ that
would bid $\bid\primed$.  Thus, the incentive inconsistency is zero.
\end{proof}

Comparing the utility of the agent for following the dashboard and
bidding $\bid\primed$ for outcome $s \in \{1,\ldots,t-1\}$ we see
that the former is the utility maximizing outcome for value $\val$
while the latter is the utility maximizing outcome for value $\val
\super s$.  Since the agent's value is $\val$ the utility of the
former is at least the utility of the latter.  For outcome $t$
(allocation from stage $t$ and payment from stage 1), the utility from
following the dashboard can be worst than the incentive compatible
utility by at most $\val$ (as the difference between the correct
payment for round $t$ and the actual payment in round 1 is at most
$\val$), and the incentive compatible utility is at least the
utility from bid $\bid\primed$.  
%
Thus, the total regret is at most $\val$ and the per-stage regret is
at most $\val/t$.

\begin{corollary}
For the all-pay last-stage dashboard mechanism, an agent with value $\val$ that follows the dashboard for $t$ stages has per-stage regret at most $\val/t$
\end{corollary}

The above analysis of incentive consistency of the
follow-the-dashboard strategy guarantees that following the dashboard
is a good strategy compared to constant-bid deviations when the agents
value is constant in each round.  This analysis does not rule out the
possibility that some other strategy is better than following the
dashboard.  In the next section we develop dashboard mechanisms that
are incentive consistent for all strategies.  Importantly, this
property enables dashboards that work even when the agents' values and
the allocation algorithm changes from stage to stage.


==> no_regret.tex <==
\section{Implementation with Learning Agents}
\label{s:no-regret}



This section considers the implementation of a social choice rule in
an iterated environment with no-regret agents.  No-regret follows from
the usual equilibrium assumptions as well as any number of standard
algorithms for online and multi-armed bandit learning.

\subsection{No-regret Dashboards}

We refer to a dashboard as being no-regret if, regardless of the
actions of other agents, the regret of an agent that follows the
dashboard vanishes.  In this section we give no-regret dashboards and
analyze the rate at which regret vanishes.  The dashboards in this
section are based on the empirical values dashboard which calculates
(\Cref{d:inferred-values-dashboard}):

\begin{enumerate}
\item The inferred valuation profile for stage $s \in \{1,\ldots,t\}$
  is $\evals \super s$.

\item The profile of single-agent allocation rules for stage $s \in
  \{1,\ldots,t\}$ is $\allocs \super s$ with $\alloci \super s (z) =
  \alloci(z,\evalsmi \super s)$ for each agent $i$.
\end{enumerate}


While our focus is on dashboards for winner-pays-bid mechanisms, to
give some intuition for how no-regret dashboards are constructed, we
first describe no-regret dashboards for all-pay mechanisms.  All-pay
mechanisms are simpler to give no-regret dashboards for as payments
are deterministic: an agent pays her bid regardless of the outcome of
the mechanism.  

\begin{definition} 
The (empirical values) {\em last-stage} dashboard at stage $t+1$ the
profile of single-agent bid allocation rules $\dallocs \super {t+1}$
that correspond to profile $\allocs \super {t}$ via
equation~\eqref{eq:single-agent-bid-allocation-rule}.
\end{definition}

A key fact about this dashboard is that an agent $i$ with value
$\vali$ that follows the dashboard in stage $t+1$ makes correct
payment for the realized allocation rule of stage $t$.  If the agent
follows the dashboard in every stage the total payments are correct
except the payments for an arbitrary allocation rule in the first
stage are swapped in for the correct payments for the last stage.  

\begin{lemma} 
The per-stage regret of an agent $i$ with value $\vali$ for following
the dashboard after stage $t$ is at most $\vali/t$.
\end{lemma}
\begin{proof}
We compare the utility of following the dashboard to any fixed bid in
hindsight.  (As usual, ``in hindsight'' means that the behavior of the
mechanism in each stage is fixed according to the actions of other
agents and the mechanism when the agent follows the dashboard.)  We
will consider grouping the allocation of stage $s$ with the payment in
stage $s+1$ (with the allocation of round $t$ paired with the payment
of round $1$) and we will refer to this grouping as outcome $s$.  As
we have argued above, if the agent follows the dashboard, outcomes
corresponding to $s \in \{1,\ldots,t-1\}$ are incentive compatible
outcomes for the allocation rule of stage $s$ and value $\vali$.  

On the other hand, if agent $i$ deviates to bid $\bidi\primed$ in
every stage, similarly grouping allocations and payments into
outcomes, the outcome in stage $s \in \{1,\ldots,t\}$ are incentive
compatible outcomes for the allocation rule of stage $s$ and the value
$\vali \super s$ that would bid $\bidi\primed$. 

Comparing the utility of the agent for following the dashboard and
bidding $\bidi\primed$ for outcome $s \in \{1,\ldots,t-1\}$ we see
that the former is the utility maximizing outcome for value $\vali$
while the latter is the utility maximizing outcome for value $\vali
\super s$.  Since the agent's value is $\vali$ the utility of the
former is at least the utility of the latter.  For outcome $t$
(allocation from stage $t$ and payment from stage 1), the utility from
following the dashboard can be worst than the incentive compatible
utility by at most $\vali$ (as the difference between the correct
payment for round $t$ and the actual payment in round 1 is at most
$\vali$), and the incentive compatibile utility is at least the
utility from bid $\bidi\primed$.  

Thus, the total regret is at most $\vali$ and the per-stage regret is
at most $\vali/t$.
\end{proof}

The approach of the last-stage dashboard can be generalized to average
over multiple past stages.  For example, the {\em sliding window}
dashboard averages the allocation rules of the past $k$ stages to
obtain the allocation rule from which the dashboard is constructed.
The per-stage regret of this dashboard is bounded by $k\vali/t$.  The
{\em geometric averaging} dashboard constructs the dashboard for stage
$t$ from the weighted average of the past stages $\{1,\ldots,t-1\}$ by
averaging stage $t-k$ with weight $2^{-k}$ and stage 1 with weight
$2^{-t+2}$ (so the total weight is 1).  A counting argument shows that
the per-stage regret is again $\vali/t$.

The approach to enforcing the no-regret property for dashboard
mechanisms is to make sure that the cumulative payments approximately
correspond to the cumulative allocation rule.  If they do, then the
characterization of Bayes-Nash equilibrium (cf.\ incentive
compatibility) implies that following the dashboard is better than any
fixed strategy in hindsight (except for in the last stage).  This
approach was fairly easy to execute with all-pay mechanisms as
payments equal bids deterministically, and thus, we can enforce that
the next stage payments are correct for the current stage.  For
winner-pays-bid mechanisms, it will not be as easy to collect payments
from future stages as these payments are only collected when the agent
wins.

A very generic approach to resolving this issue is to have the
dashboard mechanism keep track of the a balance, the amount underpaid
or overpaid by the agent according to the values inferred from bids
for past rounds.  This balance can be adjusted towards zero in future
rounds.  The regret of following the dashboard will be upper bounded
by the outstanding balance.






==> no_regret_inference.tex <==

\section{Dashboards for No-regret Learning Agents}
\label{s:no-regret}

The dashboard mechanisms described thus admit a simple approximately
optimal strategy of following the dashboard.  Agents may, however,
attempt to follow other natural strategies, and we would like to
guarantee that in these cases good outcomes arise.  A specific
candidate family of bidding strategies we would like to consider are
given by no-regret algorithms.  These algorithms guarantee performance
comparable to a single-bid in hindsight.  In this section we show
that the inference method of \citet{NST-15} for no-regret agents gives
a method for inferring the values of such agents.  Though we do not
describe the details here, with these estimated values the dashboard
can be adjusted so that good outcomes are obtained.  We will require
that the regret of an agent is non-negative and vanishing with the
number of rounds.  This property is satisfied for the usual no-regret
learning algorithms.


Next we establish properties of no-regret
learning strategies for all-pay and 
winner-pays-bid  dashboard mechanisms that 
are incentive consistent on average. Our main 
result uses the idea of rationalizable
sets for learning bidders 
developed in \citet{NST-15}. The rationalizable
set contains pairs of value and average
regret of the learning bidder that are 
compatible with the observed bid sequence.
In this section we show that under mild
condition of the strictly increasing social
choice function with its first derivative
bounded away from zero, the rationalizable
set of the learning bidder in the dashboard
mechanism is strictly convex. As result,
if this bidder has vanishing regret, the
set of values that rationalizes this bidder's
behavior shrinks around the true value
of this bidder. Therefore, the dashboard
mechanism provides a correct allocation 
to this bidder in the limit. This result is
valid both for the all-pay dashboard mechanism
and for the winner-pays-bid mechanism. We
also show that the average price that bidder 
pays in the two mechanisms approaches the optimal fixed bid in hindsight, i.e. 
minimizes regret.

\subsection{Increasing Allocation Rules Imply Concave Bid Allocation Rules}
Convexity of the rationalizable set is
related to the slope of the allocation rule
for the values.
We begin by analyzing the properties of the 
allocation rule and derive sufficient
conditions that ensure strong convexity
of the rationalizable set of a low regret
learning bidder.

As we discuss below, in general, a lower bound on the derivative of the allocation rule for
values implies a lower
bound on the second derivative of the bid-allocation rule (which is
negative because the bid allocation rule is concave).  Intuitively, the
incremental cost of additional allocation probability is increases as bidder is allocated more.

\begin{lemma} 
\label{l:strictly-monotone}
%A strict monotonicity constraint on the (value) allocation rule
%$\alloc$ is related to a bounded concavity %constraint on the
%corresponding (all-pay) bid allocation rule %$\balloc$; 
The following
are equivalent for $\delta > 0$ and an all-pay allocation rule:
$$
(i)\;\;\alloc'(\val) \geq \delta \quad\quad \mbox{and}\quad\quad (ii)\;\;
\balloc''(\price(\val)) \geq -1/\delta\val^3
$$
 where $\bid = \price(\val)$ is the bid of the agent with value
 $\val$.  The following are also equivalent
 for $\delta>0$:
$$
(i)\;\;\alloc'(\val) \geq \delta/v^3 \quad\quad \mbox{and}\quad\quad (ii)\;\;
\balloc''(\price(\val)) \geq -1/\delta
$$
\end{lemma}

\begin{proof}
To make the notation simple, let $\phi = \alloc^{-1}$ map allocation
probabilities to the values that obtain them according to $\alloc$.
Let $\Phi(\alloc) = \int_0^{\alloc}\phi(z)\,dz$ be the payment
required to receive allocation $\alloc$.  Note that $\Phi$ is the
inverse of $\balloc$, i.e., $\balloc = \Phi^{-1}$.

Now consider the implication of a lower bound on the derivative of
$\alloc$ as $\alloc'(\val) \geq \delta$.  Then $\Phi''(\alloc) =
\phi'(\alloc) \leq 1/\delta$.  Calculate $\balloc''(\price(\val)) = -
\Phi''(\alloc(\val)) / (\Phi'(\alloc(\val)))^3 = -
\Phi''(\alloc(\val)) / \val^3$ with the second inequality from noting
that $\Phi' = \phi = \alloc^{-1}$ which maps allocation probability to
values.  Thus, our inequality of $\Phi''(\alloc) \leq 1/\delta$
implies $\balloc''(\price(\val)) \geq -1/\delta \val^3$.

The second equivalence follows from the first equivalence by substitution.
\end{proof}

We can provide an parallel lemma that applies
to a winner-pays-bid allocation rule.
\begin{lemma} 
\label{l:strictly-monotone:fpa}
The following
are equivalent for $\delta > 0$ and a winner-pays-bid allocation rule:
$$
(i)\;\;\alloc'(\val) \geq \delta \quad\quad \mbox{and}\quad\quad (ii)\;\;
\balloc''(\price(\val)) \geq -1/\delta\val^3
$$
 where $\bid = \price(\val)$ is the bid of the agent with value
 $\val$.  The following are also equivalent
 for $\delta>0$:
$$
(i)\;\;\alloc'(\val) \geq \delta/v^3 \quad\quad \mbox{and}\quad\quad (ii)\;\;
\balloc''(\price(\val)) \geq -1/\delta
$$
\end{lemma}
\begin{proof}
As in the analysis of the all-pay mechanism, let $\phi = \alloc^{-1}$ map allocation
probabilities to the values that obtain them according to $\alloc$.
Let $\Phi(\alloc) = \int_0^{\alloc}\phi(z)\,dz$ be the payment
required to receive allocation $\alloc$. Then the price that bidder pays is $b(x)=\frac{\Phi(\alloc)}{\alloc}$. 
Note that $b(\cdot)$ is the
inverse of $\balloc$, i.e., $\balloc = b^{-1}$.

Now consider the implication of a lower bound on the derivative of
$\alloc$ as $\alloc'(\val)/\alloc(\val) \geq \delta$.  Then $
\alloc \phi'(\alloc) \leq 1/\delta$.
Note that 
$$
\balloc'(\price(v))=\frac{1}{b'(x(v))}=\frac{x(v)}{v-b(x(v))}.
$$
Then 
$$
\balloc''(\price(v))=-
\frac{b''(x(v))}{(b'(x(v))^3}=
-\frac{x^2}{(\val-b)^3}[\phi'/x-2(\val-b)/x^2] \geq
-\frac{x^2 \phi'}{(\val-b)^3} \geq -\frac{1}{\delta \val^3}.
$$


The second equivalence follows from the first equivalence by substitution.
\end{proof}


\begin{lemma}
\label{l:concavity-and-sum}
If the second derivative of $\balloc \super s$ for $s \in\{1,\ldots,t\}$ is at least $-1/\delta$, then so 
is the second derivative of 
$\frac{1}{t}\sum_s \balloc \super s$.
\end{lemma}


\begin{lemma}
\label{l:preservation-of-strict-allocation}
For stage (value) allocation rule $\alloc \super s$ for $s
\in\{1,\ldots,t\}$ and the corresponding bid allocation rules $\balloc \super
s$ consider the average bid allocation rule $\balloc = \frac{1}{t} \sum_{s \leq t} \balloc
\super s$, and (value) allocation rule $\alloc$ resulting from
$\balloc$. Then if each $\alloc \super s$ for $s \leq t$ has the first derivative of least $\delta/\val^3$ at
$\val$ then so does $\alloc$.
\end{lemma}

\begin{proof}
Apply \Cref{l:strictly-monotone} and \Cref{l:concavity-and-sum} and then apply \Cref{l:strictly-monotone} again.
\end{proof}.

\begin{lemma}\label{lemma:fixed:bid}
If the stage (value) allocation rules that are strictly monotone with
derivative at least $\delta/\val^3$ then the utility function induced
by single best-in-hindsight bids (in the all-pay stage mechanisms) is
$1/\sqrt{\delta}$-strongly convex.
\end{lemma}

\begin{proof}
Best-in-hindsight bidding strategies are incentive consistent on
average.  Thus, the average outcome for a fixed bid is equivalent to
the average of the all-pay stage mechanisms outcome for the bid.
Thus, \Cref{l:preservation-of-strict-allocation} implies strict
monotonicity of the induced value allocation rule which implies strict
convexity of the utility function (the integral of the value
allocation rule).
\end{proof}


Notice that the assumption that $\alloc'(\val) \geq \delta/\val^3$ is
satisfied when values are bounded away from zero, e.g., to $[h,1]$ and
then $\alloc'(\val) \geq \delta$ is sufficient to imply $\alloc'(\val)
\geq \delta/\val^3$. The result for the winner-pays-bid mechanism is derived
identically to the result for the all-pay mechanism.
%\jc{I'm not sure this is the best way to do
%  this.  It's the first thing that came to %mind.  Also, I'm a bit
%  confused by the bound, as obviously any %result we get should be
%  scale invariant, so this should give the %same bound up to scaling as
%  if values are on $[1/h,1]$, but there we'd %need the derivative to be
%  at least $\delta h^3$ which seems to be off %by a factor of $h^2$.}

\subsection{No-regret Analysis for all-pay mechanisms}
Suppose that bidder $i$ in the dashboard mechanism with all-pay payment rule and which is incentive consistent on average uses no-regret
learning algorithm to submit bids. We can write the average regret of
this bidder at round $t$ as
$$
\Regret_i^{(t)}(b;\vali)=\vali\frac{1}{t}\sum\limits_{s \leq t}\balloci^{(s)}(b)-b
-\vali \frac{1}{t}\sum\limits_{s \leq t}\balloci^{(s)}(\bidi^{(s)})+\frac{1}{t}\sum\limits_{s \leq t}\bidi^{(s)}.
$$
The history of bids for the agent that uses a learning algorithm with bounded average regret
allows us to constrain the set of feasible pairs of value and average regret for this agent to form her rationalizable set
$$
\NRi=\left\{(\vali,\epsilon_i) \in \reals_+ \times \reals\;:\; \mbox{Regret}_i^{(t)}(b;\vali) \leq \regreti,\;\forall\, b \in \reals_+\right\}.
$$

Now we characterize the rationalizable set in the following lemma.

\begin{lemma}\label{RS:boundary}
Suppose that the dashboard mechanism is incentive consistent on average.
Also suppose that allocation rule $\alloci(\cdot)$ is differentiable with respect to $v_i$ for each $\evalsmi \in \reals_+^{n-1}$ with\\ $\inf\limits_{\evalsmi \in \reals^{n-1}_+}\frac{\partial}{\partial z} \alloci(z,\evalsmi)\vert_{z=v}\geq 1/(\alpha^2v^3)$ for some $\alpha>0$.
Then 
\begin{itemize}
    \item[(i)] The rationalizable set $\NRi \super t$ recovered at each step $t$ is $\alpha$-strongly convex;
    \item[(i)] The boundary of the rationalizable set $\NRi \super t$ is the parametric curve 
    $$
    \vali(b)=1
    \bigg/
    \frac{1}{t}\sum\limits_{s \leq t} \balloci^{\prime (s)}(b) ,\;\;\regreti(b)=
    \Regret_i^{(t)}(b;\vali(b)),\;\;b \in \reals_+
    $$
\end{itemize}
\end{lemma}


\begin{proof}
Statement (i) of the lemma follows from
Lemma \ref{lemma:fixed:bid}. In fact, convexity of the rationalizable set 
is determined by the term
$$
\vali\frac{1}{t}\sum\limits_{s \leq t}\balloci^{(s)}(b)-b,
$$
which is the utility from the fixed bid in
hindsight (since the last term is linear
in the value). By Lemma \ref{lemma:fixed:bid}
the utility from the fixed bid in hindsight is
strongly convex.

Statement (ii) is the consequence of $\NRi \super t$ being the envelope of half-spaces
$$
\regreti \geq \vali \frac{1}{t}\sum\limits_{s \leq t}\balloci^{(s)}(b)-b-
\vali\frac{1}{t}\sum\limits_{s \leq t}\balloci^{(s)}(\bidi^{(s)})+\sum\limits_{s \leq t}\bidi^{(s)}
$$
The half-space that has a common point with
the set $\NRi$ for value $\vali$ is the one
that corresponds to the smallest $\regreti$,
which is attained at the bid $b$ with
\begin{equation*}
 \vali \frac{1}{t}\sum\limits_{s \leq t}\balloci^{\prime(s)}(b)-1=0. \qedhere
\end{equation*}
\end{proof}

Next we summarize the properties of the 
inferred values of learning bidders
and their average bid when they participate
in the all-pay dashboard mechanism which is incentive consistent on average.


\begin{theorem}
\label{thm:avebidbound}
Suppose that a given player $i$ in the dashboard mechanism with an all-pay payment rule
and the allocation rule with derivative of
at least $1/(\alpha^2v^3)$ which is incentive
consistent on average and where bidder 
has regret within $[0,\,\overline{\regreti}]$.
Then 
\begin{enumerate}
\item The rationalizable values are within
$[v_i \pm 2\overline{\regreti}/\alpha]$, i.e.
if the average regret $\overline{\regreti}$
is decreasing, then the mechanism allocates
correctly for this bidder in the limit.
\item The average bid (corresponding
to the average payment in the all-pay mechanism) is bounded by
$$
\left|
\overline{\bidi^{(t)}}-\frac{1}{t}\sum\limits_{s \leq t}\bidi^{(s)}
\right| \leq \overline{\regreti}\left(
1+\frac{\alpha}{(v_i
-\overline{\regreti}/\alpha)^2}
\right)
$$
from the optimal fixed bid in hindsight $\overline{\bidi^{(t)}}$. I.e. if the average regret $\overline{\regreti}$
is decreasing, then the average payment
in the mechanism in the limit minimizes
regret of the bidder.
\end{enumerate}
\end{theorem}

\noindent The proofs of \Cref{thm:avebidbound} and \Cref{thm:avepayminreg} (below) are moved to \Cref{a:proofs}.

 
\subsection{No-regret Analysis for winner-pays-bid mechanisms}
\input{regret_FPA}




==> persuadable.tex <==
\section{Implementation with Dashboard Mechanisms}

\label{s:dashboards}


This section conducts a theoretical study of a practical approach to
bidding and optimization in Internet markets.  The principal publishes
a bidding dashboard which informs the agents of the market conditions;
the agents use this dashboard to optimize their bids.  We consider
dashboards that give each agent estimates of the outcome of the
mechanism any possible bid of the agent.  These estimates can be
constructed, for example, from historical bid behavior of the agents
in the mechanism.

\begin{definition}
A {\em dashboard} $\dallocs \in (\reals \to [0,1])^n$ for an $n$-agent
winner-pays-bid mechanism is a profile of $n$ bid-allocation rules
$\dallocs = (\dalloci[1],\ldots,\dalloci[n])$ where $\dalloci(\bid)$
is the forecasted probability that agent $i$ wins with bid $\bid$.
\end{definition}


Our perspective is that the principal has more information than the
agents about counterfactual outcomes in the mechanism, i.e., what would
have happened if an agent had made a different bid in the past.
However, the principal does not have perfect information about the
future nor does the principal attempt to predict changing actions of
agents due to changes in preferences or strategic behavior.  Thus, it
is impossible for the principal to always give accurate advice to the
agents by the way of a bidding dashboard.  Motivated by this situation
we consider the following definition that describes agents that are
willing to follow the advice of a principal who is learning how to
give good advice.

\begin{definition}
\label{d:persuadable}
A {\em persuaded} agent bids according to the dashboard.  If bidding
according to the dashboard converges to a best response, a {\em
  persuadable} agent is persuaded.  A dashboard mechanism {\em implements
an outcome for persuadable agents} if bidding according to the
dashboard (i) converges to a Nash equilibrium and (ii) the outcome of
this Nash equilibrium is the desired outcome.
\end{definition}


We consider the implementation for persuadable agents of a strictly
monotone and continuously differentiable social choice function
$\allocs : \reals^n \to [0,1]^n$ by dashboard mechanisms.  We
consider two design questions: (a) what dashboard should the principal
publish and (b) what mechanism should the principal run.  For the
mechanism to implement the social choice function for persuadable
agents, it must satisfy properties (i) and (ii) of
Definition~\ref{d:persuadable}.  In fact, if agents are persuaded by
the dashboard, then the mechanism to implement the social choice
function is straightforward.

\begin{definition}
\label{d:dashboard-mechanism}
The winner-pays-bid dashboard mechanism $\ballocs : \reals^n \to
[0,1]^n$ for dashboard $\dallocs$ and social choice function $\allocs$
is:
\begin{enumerate}
\item[0.] Solicit bids $\bids$ for dashboard $\dallocs$.
\item \label{s:dashboard-inference} Infer values $\evals$ from bids
  from equation~\eqref{eq:single-agent-foc} as $\evali = \bidi +
  \dalloci(\bidi) / \dalloci'(\bidi)$ for each $i$.
\item Output allocation $\ballocs = \allocs(\evals)$ (with prices $\bprices$ as $\bpricei = \bidi\,\balloci$).
\end{enumerate}
\end{definition}

Notice that in the above definition the bid allocation rule $\ballocs$
is a mapping $\reals^n \to [0,1]^n$ from bid profiles to allocation
profiles while the dashboard is a profile of single-agent bid
allocation rules $(\reals \to [0,1])^n$ each of which maps a bid to a
probability of winning.  In other words, outcomes according to the
dashboard are calculated independently across the agents while
outcomes according to the mechanism depend on the reports of all
agents together.  The following proposition follows simply from the
correctness of equation~\eqref{eq:single-agent-foc}.

\begin{prop} 
The dashboard mechanism (\Cref{d:dashboard-mechanism}) for any given strictly monotone and
continuously differentiable dashboard and social choice function
implements the social choice function if agents are persuaded.
\end{prop}

We consider the dashboard mechanism for a given social choice function
in an iterated environment with agents with persistent values, i.e.,
that are unchanging over each iteration.  In practice these iterations
could correspond to a new user arriving in the market to be matched
with the agents or an aggregation of such arrivals over, e.g., one
billing cycle of the agents.  In this environment, the principal is
able to tune the dashboard $\dallocs$ employed with the dashboard
mechanism of \Cref{d:dashboard-mechanism}.  Notice that
changing the dashboard changes the definition of the mechanism; thus
the game played in each stage is not the same game.  The question we
address next is how the principal should construct the dashboard to
ensure the outcome for persuadable agents converges to a Nash
equilibrium and they are persuaded.

Our approach is motivated by the solution concept of fictitious play.
In fictitious play agents best respond to the empirical distribution
of the actions in previous rounds.  Fictitious play assumes that the
agents know the actions in past rounds.  The principal could publish
these actions; however, a better approach is to just publish as a
dashboard the aggregate bid allocation rules that result.  Our
dashboard follows this approach except with respect to estimated
values rather than actions.  Best responding to such a dashboard is,
in a sense, an improvement on fictitious play.


\begin{definition}
\label{d:inferred-values-dashboard}
For stage $t+1 \geq 2$, the {\em inferred values dashboard} is the
profile of single-agent bid allocation rules $\dallocs \super {t+1}$
defined as follows:
\begin{enumerate}
\item The inferred valuation profile for stage $s \in \{1,\ldots,t\}$ is $\evals \super s$.

\item The profile of single-agent allocation rules for stage $s \in \{1,\ldots,t\}$ is $\allocs \super s$ with $\alloci \super s (z) = \alloci(z,\evalsmi \super s)$ for each agent $i$.
\item The empirical profile of single-agent allocation rules at stage $t+1$ is $\eallocs \super {t+1}$ with $\ealloci \super {t+1} (z) = \frac{1}{t} \sum_{s\leq t} \alloci \super s (z)$ for each agent $i$.
\item 
The estimated values dashboard is the profile of single-agent bid
allocation rules $\dallocs \super {t+1}$ that correspond to profile
$\eallocs \super {t+1}$ via
equation~\eqref{eq:single-agent-bid-allocation-rule}.
\end{enumerate}
\end{definition}


We now prove the rather straightforward result that the dashboard
mechanism (\Cref{d:dashboard-mechanism}) with the inferred
values dashboard (\Cref{d:inferred-values-dashboard})
converges to a Nash equilibrium and the outcome of this Nash
equilibrium is that of the social choice rule.  In fact, it converges
in round two.  The dashboard $\dallocs \super 1$ used in stage~1 can
be any continuous and strictly monotone profile of bid allocation
rules.
\newpage

\begin{theorem}
For any fixed valuation profile $\vals$ and any continuous and
strictly monotone social choice function $\allocs$, the dashboard
mechanism %(Definition~\ref{d:dashboard-mechanism}) 
with the inferred
values dashboard %(Definition~\ref{d:inferred-values-dashboard}) 
converges to a
Nash equilibrium.  Specifically, given that agents are persuaded by
the dashboard up to and including round $t \geq 1$, bids in round $t+1
\geq 2$ are in Nash equilibrium.
\end{theorem}

\begin{proof}
The dashboards up to and including round $t$ are the average of the
bid allocation rule for a continuous and strictly increasing social
choice function; thus they are continuous and strictly increasing.  By
equation~\eqref{eq:single-agent-foc} the inferred values of persuaded
agents are the true values.  These values are the same in each stage;
thus the profile of single-agent allocation rules in each stage is the
one that corresponds to the social choice function on true valuation
profile.  The average of these profiles of allocation rule is the
profile itself (they are all the same).  The dashboard is the
corresponding profile of single-agent bid allocation rules.

Consider agent $i$ and assume that other agents are persuaded in stage
$t+1$.  Thus, the estimated profile of other agent values is
$\evalsmi\super{t+1} = \valsmi$.  The allocation rule in value space
faced by agent $i$ is $\alloci \super {t+1} (z) = \alloci(z,\valsmi)$
which is equal to the allocation rule in all the previous stages.  As
the dashboard suggests bidding optimally according to the allocation
rule of the previous stages, bidding according to the dashboard is
agent $i$'s best response.  Persuasion is a Nash equilibrium in stage
$t+1$.
\end{proof}

The dashboard mechanism proposed in this section is simple and
practical and can implement any strictly monotone and continuously
differentiable social choice function.  For example welfare
maximization with a convex regularizer gives such a social choice
function.  For the paradigmatic problem of single-minded combinatorial
auction environments, our dashboard mechanism with the regularized
welfare-maximization social choice function gives outcomes that can be
arbitrarily close to optimal (for the appropriate regularizer).


==> regret_FPA.tex <==
Now we consider winner-pays-bid mechanism
in which the bidders use low average
regret learning algorithms and provide
results analogous to those that we produced
for the all-pay mechanism.
Suppose that bidder $i$ in the dashboard mechanism uses no-regret
learning algorithm to submit bids. We can write the average regret of
this bidder at round $t$ as
$$
\Regret_i^{(t)}(b;\vali)=\frac{1}{t}\sum\limits_{s \leq t}\balloci^{(s)}(b)(\vali-b)-
\frac{1}{t}\sum\limits_{s \leq t}\balloci^{(s)}(\bidi^{(s)})(\vali-\bidi^{(s)}).
$$
Now we describe the properties of the rationalizable set for this bidders in 
this mechanism.

\begin{lemma}\label{RS:boundary:FPA}
Suppose that the dashboard mechanism is incentive consistent on average.
Also suppose that allocation rule $\alloci(\cdot)$ is differentiable with respect to $v_i$ for each $\evalsmi \in \reals_+^{n-1}$ with\\ $\inf\limits_{\evalsmi \in \reals^{n-1}_+}\frac{\partial}{\partial z} \alloci(z,\evalsmi)/
\alloci(z,\evalsmi)\vert_{z=v}\geq 1/(\alpha^2v^3)$ for some $\alpha>0$.
Then 
\begin{itemize}
    \item[(i)] The rationalizable set $\NRi \super t$ recovered at each step $t$ is $\alpha$-strongly convex;
    \item[(i)] The boundary of the rationalizable set $\NRi \super t$ is the parametric curve 
    $$
    \vali(b)=b + \frac{1}{t}\sum\limits_{s \leq t}\balloci \super s (b)
    \bigg/
    \frac{1}{t}\sum\limits_{s \leq t} \balloci^{\prime (s)}(b) ,\;\;\regreti(b)=
    \Regret_i^{(t)}(b;\vali(b)),\;\;b \in \reals_+
    $$
\end{itemize}
\end{lemma}


\begin{proof}
Statement (i) of the lemma follows from
the analog of Lemma \ref{lemma:fixed:bid}
for the first-price auctions. In fact, given that the second term is linear in the value
of the bidder, convexity properties
of the rationalizable set are determined solely by the first term. The first term
is the utility of the bidder from the 
fixed bid in hindsight. Strong convexity
of this utility implies strong convexity of
the rationalizable set.



Statement (ii) is the consequence of $\NRi \super t$ being the envelope of half-spaces
\begin{equation*}
\regreti \geq \vali \frac{1}{t}\sum\limits_{s \leq t}\balloci^{(s)}(b)-b\frac{1}{t}\sum\limits_{s \leq t}\balloci^{(s)}(b)-
\frac{1}{t}\sum\limits_{s \leq t}\balloci^{(s)}(\bidi^{(s)})(\vali-\bidi^{(s)})
\qedhere
\end{equation*}
\end{proof}


Next we provide the summary result that 
ensures that for learning bidders with 
vanishing regret, the dashboard mechanism
that is incentive compatible on average
allocates correctly in the limit and the 
average payment of the learning bidders
minimizes their regret.


\begin{theorem}
\label{thm:avepayminreg}
Suppose that a given player in the dashboard mechanism with a winner-pays-bid payment rule
and the allocation rule with log-derivative of
at least $1/\alpha^2v^3$ which is incentive
consistent on average and where bidder 
has regret within $[0,\,\overline{\regreti}]$.
Then 
\begin{enumerate}
\item The range of values that rationalizes
bids of this bidder is contained in $[v_i \pm 2 \overline{\regreti}/\alpha]$. In other words, if the bidder has vanishing regret, then the mechanism allocates this bidder
correctly in the limit.
\item The average payment per unit of allocation can be bounded as
$$
\left|
\overline{\bidi^{(t)}}-\frac{\frac{1}{t}\sum\limits_{s \leq t}\bidi \super s \balloci \super s (\bidi \super s)}
 {\frac{1}{t}\sum\limits_{s \leq t}\balloci \super s (\bidi \super s)}
\right| \leq \frac{\overline{\regreti}}{
\alpha^2v_i-\alpha\overline{\regreti}}\left(
1+\frac{\alpha^3}{v_i
-\overline{\regreti}/\alpha}
\right)
$$
from the optimal fixed bid in hindsight $\overline{\bidi^{(t)}}$. In other words,
the average payment of this bidder in the 
limit minimizes regret.
\end{enumerate}
\end{theorem}



